Deep learning for CALPHAD modeling: Universal parameter learning solely based on chemical formula

Empowering the creation of thermodynamic and property databases, the CALPHAD (CALculation of PHAse Diagrams) methodology plays a vital role in enhancing materials and manufacturing process design. In this study, we propose a deep learning approach to train parameters in CALPHAD models solely based on chemical formula. We demonstrate its application through an example of calculating the mixing parameter of liquids. This work showcases the integration of CALPHAD and deep learning, highlighting its potential for achieving automated comprehensive CALPHAD modeling.

==> backup/ds-revision-tools-202107.tex <==
% Works for PRB
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% my commenting setup
\usepackage[textsize=footnotesize, textwidth=1.4cm, backgroundcolor=yellow]{todonotes}%\reversemarginpar
\makeatletter
% Don't know why but the customization below did not work for aastex.
\renewcommand{\todo}[2][]{%
    \@todo[caption={#2}, #1]{#2}%
}
% if the above does not work. 
%\renewcommand{\todo}[2][]{%
%    \@todo[caption={#2}, #1]{\renewcommand{\baselinestretch}{0.3}\scriptsize#2}%
%} 
\newcommand{\inlinecomment}[1]{\todo[color=yellow!30, inline]{#1\par}\noindent}
\newcommand{\urgentcomment}[1]{\todo[color=red!30, inline]{[URGENT] #1\par}\noindent}
\newcommand{\resolvedcomment}[1]{\todo[color=blue!10, inline]{[Resolved] #1\par}\noindent}
\newcommand{\sidecomment}[1]{\todo[color=yellow!30,linecolor=red, size=\tiny]{#1\par}}
\newcommand{\urgentsidecomment}[1]{\todo[color=red!30, linecolor=red, size=\tiny]{[URGENT] #1\par}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% writing help
\newcommand{\resume}{\colorbox{pink}{\textbf{--- Resume writing from here ---}}}
\newcommand{\addrefs}{\colorbox{yellow}{[add refs]}}
\newcommand{\fillout}{\colorbox{yellow}{[xxx]}}
\newcommand{\yhl}[1]{\colorbox{yellow}{#1}}
%\usepackage{comment}
%\usepackage{listings} % write latex command
% changes should come after todonotes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% writing help
%\usepackage{comment}
\usepackage{listings} % write latex command


==> ds-revision-tools-202107.tex <==
% Works for PRB
%%%%%%%%%%%%%%%%%%%%%%%%%%%
% my commenting setup
\usepackage[textsize=footnotesize, textwidth=1.4cm, backgroundcolor=yellow]{todonotes}%\reversemarginpar
\makeatletter
% Don't know why but the customization below did not work for aastex.
\renewcommand{\todo}[2][]{%
    \@todo[caption={#2}, #1]{#2}%
}
% if the above does not work. 
%\renewcommand{\todo}[2][]{%
%    \@todo[caption={#2}, #1]{\renewcommand{\baselinestretch}{0.3}\scriptsize#2}%
%} 
\newcommand{\inlinecomment}[1]{\todo[color=yellow!30, inline]{#1\par}\noindent}
\newcommand{\urgentcomment}[1]{\todo[color=red!30, inline]{[URGENT] #1\par}\noindent}
\newcommand{\resolvedcomment}[1]{\todo[color=blue!10, inline]{[Resolved] #1\par}\noindent}
\newcommand{\sidecomment}[1]{\todo[color=yellow!30,linecolor=red, size=\tiny]{#1\par}}
\newcommand{\urgentsidecomment}[1]{\todo[color=red!30, linecolor=red, size=\tiny]{[URGENT] #1\par}}
\makeatother
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% writing help
\newcommand{\resume}{\colorbox{pink}{\textbf{--- Resume writing from here ---}}}
\newcommand{\addrefs}{\colorbox{yellow}{[add refs]}}
\newcommand{\fillout}{\colorbox{yellow}{[xxx]}}
\newcommand{\yhl}[1]{\colorbox{yellow}{#1}}
%\usepackage{comment}
%\usepackage{listings} % write latex command
% changes should come after todonotes
%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% writing help
%\usepackage{comment}
\usepackage{listings} % write latex command

